Instantaneous convective heat transfer at the wall: a depiction of turbulent boundary layer structures

We demonstrate the ability to experimentally measure fluctuations of the convective heat transfer coefficient at the wall in a turbulent boundary layer. For this, we measure two-dimensional fields of wall-temperature fluctuations beneath a zero-pressure-gradient turbulent boundary layer, at two moderate friction Reynolds numbers ($Re_\tau \approx 990$ and $Re_\tau \approx 1800$). Spatiotemporal data of wall-temperature are acquired by means of a heated-thin-foil sensor as sensing hardware, and an infrared camera as temperature detector. At low $Re_\tau$ conditions, the fields of the Nusselt number fluctuations are populated by elongated structures comprising streamwise and spanwise length scales comparable to those of near-wall streaks. At higher $Re_\tau$ conditions, the effective width and length of the coherent $Nu$ fluctuations increases. These findings are based on two-point correlations, as well as streamwise-spanwise energy spectra of $Nu$ fluctuations. The convective velocities of the $Nu$ fluctuations are also computed with the available time resolution from the measurements. This allows for resolving the multi-scale nature of convective footprints of wall-bounded turbulence: our experimental data reflect that larger streaks in the footprint convect at velocities in the order of the free-stream velocity, while the more energetic smaller-scale features move at velocities in the order of $10u_\tau$. Measurements of the kind presented here offer a promising method for sensing, as they can be used as input to flow control systems.

==> Sections/Nomenclature.tex <==
\nomenclature{$Re_{\tau}$}{friction Reynolds number}
\nomenclature{$Re_{\Theta}$}{momentum Reynolds number}
\nomenclature{$U_\infty$}{free-stream velocity}
\nomenclature{$u_{\tau}$}{friction velocity}
\nomenclature{$\tau_w$}{wall skin friction}
\nomenclature{$\rho$}{density}
\nomenclature{$\nu$}{kinematic viscosity}
%\nomenclature{$\beta$}{Rotta-Clauser pressure-gradient parameter}
\nomenclature{$\delta_{99}$}{boundary layer thickness}
%\nomenclature{$\delta^*$}{displacement thickness}
%\nomenclature{$H$}{shape factor}
\nomenclature{$\dot{q}_{in}$}{Joule heat flux}
\nomenclature{$\dot{q}_{rd}$}{radiation heat flux}
\nomenclature{$\dot{q}_{cd}$}{lateral conduction heat flux}
\nomenclature{$B$}{temporal delay}
\nomenclature{$I$}{current intensity}
\nomenclature{$V$}{electric voltage}
\nomenclature{$A$}{foil surface area}
\nomenclature{$\epsilon$}{emissivity}
\nomenclature{$\sigma$}{Stefan-Boltzmann constant}
\nomenclature{$T_w$}{wall temperature}
\nomenclature{$T_{aw}$}{adiabatic wall temperature}
\nomenclature{$k$}{thermal conductivity}
\nomenclature{$\delta_f$}{foil thickness}
\nomenclature{$\delta_p$}{paint layer thickness}
\nomenclature{$l^+$}{characteristic length}
%\nomenclature{$Bi$}{Biot number}
\nomenclature{$h$}{convective heat transfer coefficient}
\nomenclature{$c$}{specific heat}
\nomenclature{$Nu$}{Nusselt number}
\nomenclature{$y^+$}{TBL inner unit}
%\nomenclature{$C$}{effective thermal conductivity}
%\nomenclature{$P$}{pressure}
\nomenclature{$U_c$}{convective velocity}
\nomenclature{$\omega$}{frequency}
\nomenclature{$k_x$}{wave-number in flow direction}
\nomenclature{$t$}{time}

\begin{figure}
    \centering
    \begin{mdframed}
        \begin{multicols}{2}
            \printnomenclature
        \end{multicols}
    \end{mdframed}
\end{figure}

==> references.tex <==
% This is jfm2esam.bib v1.0 08/14/02
%
@book{astarita2012infrared,
  title={Infrared thermography for thermo-fluid-dynamics},
  author={Astarita, T. and Carlomagno, G. M.},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{howard1982narcissus,
  title={Narcissus: reflections on retroreflections in thermal imaging systems},
  author={Howard, J. W. and Abel, I. R.},
  journal={Appl. Optics},
  volume={21},
  number={18},
  pages={3393--3397},
  year={1982},
  publisher={Optica Publishing Group}
}

@Article{chauhan:2009a,
  author = 	 {K. A. Chauhan and P. A. Monkewitz and H. M. Nagib},
  title = 	 {Criteria for assessing experiments in zero pressure gradient boundary layers},
  journal =  {Fluid Dyn. Res.},
  year = 	 2009,
  volume =	 41,
  number =	 {},
  pages =	 {},
  note =     {021404},
}

@article{meola2015measurements,
  title={Measurements of very small temperature variations with LWIR QWIP infrared camera},
  author={Meola, C. and Boccardi, S. and Carlomagno, G. M.},
  journal={Infrared Phys. Techn.},
  volume={72},
  pages={195--203},
  year={2015},
  publisher={Elsevier}
}

@article{gu2024denoising,
  title={Denoising image-based experimental data without clean targets based on deep autoencoders},
  author={Gu, F. and Discetti, S. and Liu, Y- and Cao, Z. and Peng, D.},
  journal={Exp. Therm. Fluid Sci.},
  volume={156},
  pages={111195},
  year={2024},
  publisher={Elsevier}
}

@article{winterton1998did,
  title={Where did the {D}ittus and {B}oelter equation come from?},
  author={Winterton, R. H. S.},
  journal={Int. J. Heat Mass Tran.},
  volume={41},
  number={4-5},
  pages={809--810},
  year={1998},
  publisher={Pergamon}
}

@article{marusic2019attached,
  title={Attached eddy model of wall turbulence},
  author={Marusic, I. and Monty, J. P},
  journal={Annu. Rev. Fluid Mech.},
  volume={51},
  number={1},
  pages={49--74},
  year={2019},
  publisher={Annual Reviews}
}

@article{pirozzoli2016passive,
  title={{Passive scalars in turbulent channel flow at high {R}eynolds number}},
  author={S. Pirozzoli and M. Bernardini and P. Orlandi},
  journal={J. Fluid Mech.},
  volume={788},
  pages={614--639},
  year={2016},
  publisher={Cambridge University Press}
}

@article{alcantara2021directjfm,
  title={Direct numerical simulation of thermal channel flow for {Re}$_\tau$= 5000
  and {Pr}=0.71},
  author={Alc{\'a}ntara-{\'A}vila, F. and Hoyas, S. and P{\'e}rez-Quiles, M. J.},
  journal={J. Fluid Mech.},
  volume={916},
  pages={A29},
  year={2021},
  publisher={Cambridge University Press}
}

@article{alcantara2021direct,
  title={{Direct numerical simulation of thermal channel flow for medium--high Prandtl numbers up to {Re}$_\tau$= 2000}},
  author={Alc{\'a}ntara-{\'A}vila, Francisco and Hoyas, Sergio},
  journal={Int. J. Heat Mass Tran.},
  volume={176},
  pages={121412},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{iritani1985heat,
  title={Heat transfer mechanism and associated turbulence structure in the near-wall region of a turbulent boundary layer},
  author={Iritani, Y. and Kasagi, N. and Hirata, M.},
  booktitle={Turbulent Shear Flows 4: Selected Papers from the Fourth International Symposium on Turbulent Shear Flows, University of Karlsruhe, Karlsruhe, FRG, September 12--14, 1983},
  year={1983},
  pages={223--234},
  organization={Springer}
}

@article{kong2000direct,
  title={Direct numerical simulation of turbulent thermal boundary layers},
  author={Kong, Hojin and Choi, Haecheon and Lee, Joon Sik},
  journal={Phys. Fluids},
  volume={12},
  number={10},
  pages={2555--2568},
  year={2000},
  publisher={American Institute of Physics}
}

@article{perry1976experimental,
  title={An experimental study of turbulent convective heat transfer from a flat plate},
  author={Perry, AE and Hoffmann, PH},
  journal={J. Fluid Mech.},
  volume={77},
  number={2},
  pages={355--368},
  year={1976},
  publisher={Cambridge University Press}
}

@article{Gurka2004,
  title = {Detecting coherent patterns in a flume by using PIV and IR imaging techniques},
  volume = {37},
  ISSN = {1432-1114},
  DOI = {10.1007/s00348-004-0805-3},
  number = {2},
  journal = {Exp. Fluids},
  publisher = {Springer Science and Business Media LLC},
  author = {Gurka,  Roi and Liberzon,  Alex and Hetsroni,  Gad},
  year = {2004},
  month = apr,
  pages = {230–236}
}

@article{Antonia1988,
  title={Correlation between the longitudinal velocity fluctuation and temperature fluctuation in the near-wall region of a turbulent boundary layer},
  author={Antonia, R. A. and Krishnamoorthy, L. V. and Fulachier, L.},
  journal={Int. J. Heat Mass Transf.},
  volume={31},
  number={4},
  pages={723--730},
  year={1988},
  publisher={Elsevier}
}

@article{Meinders1999,
  title = {Experimental Study of the Local Convection Heat Transfer From a Wall-Mounted Cube in Turbulent Channel Flow},
  volume = {121},
  ISSN = {1528-8943},
  DOI = {10.1115/1.2826017},
  number = {3},
  journal = {J. Heat Transf.},
  publisher = {ASME International},
  author = {Meinders,  E. R. and Hanjalic,  K. and Martinuzzi,  R. J.},
  year = {1999},
  month = aug,
  pages = {564–573}
}

@article{cuellar2024measuring,
  title={Measuring time-resolved heat transfer fluctuations on a heated-thin foil in a turbulent channel airflow},
  author={Cu{\'e}llar, A. and Amico, E. and Serpieri, J. and Cafiero, G. and Baars, W. J. and Discetti, S. and Ianiro, A.},
  journal={arXiv preprint arXiv:2410.12778},
  year={2024}
}

@article{gurka2004detecting,
  title={{Detecting coherent patterns in a flume by using PIV and IR imaging techniques}},
  author={Gurka, R. and Liberzon, A. and Hetsroni, G.},
  journal={Exp. Fluids},
  volume={37},
  pages={230--236},
  year={2004},
  publisher={Springer}
}

@article{hetsroni1994heat,
  title={Heat transfer to a liquid—solid mixture in a flume},
  author={G. Hetsroni and R. Rozenblit},
  journal={Int. J. Multiphas. Fl.},
  volume={20},
  number={4},
  pages={671--689},
  year={1994},
  publisher={Elsevier}
}

@article{kim2020prediction,
  title={Prediction of turbulent heat transfer using convolutional neural networks},
  author={Kim, J. and Lee, C.},
  journal={J. Fluid Mech.},
  volume={882},
  pages={A18},
  year={2020},
  publisher={Cambridge University Press}
}

@inproceedings{reynolds1874extent,
  title = {On the extent and action of the heating surface of steam boilers},
  author = {Reynolds, O.},
  booktitle = {Proceedings of the Manchester Literary and Philosophical Society},
  volume = {14},
  year = {1874},
  note = {Session 1874-1875}
}

@article{reynolds1961extent,
  title={On the extent and action of the heating surface of steam boilers},
  author={Reynolds, O.},
  journal={Int. J. Heat Mass Tran.},
  volume={3},
  number={2},
  pages={163--166},
  year={1961},
  publisher={Pergamon}
}

@article{liu2019measurements,
  title={{Measurements of the wall-shear stress distribution in turbulent channel flow using the micro-pillar shear stress sensor MPS3}},
  author={Liu, Y. and Klaas, M. and Schr{\"o}der, W.},
  journal={Exp. Therm. Fluid Sci.},
  volume={106},
  pages={171--182},
  year={2019},
  publisher={Elsevier}
}

@inproceedings{amili2013characterization,
  title={Characterization of structures associated with low-and high-shear regions in experimental and numerical turbulent channel flows},
  author={Amili, O. and Mizuno, Y. and Buchmann, N. A and Atkinson, C. and Soria, J.},
  booktitle={Eighth International Symposium on Turbulence and Shear Flow Phenomena},
  year={2013},
  organization={Begel House Inc.}
}

@article{amili2011film,
  title={A film-based wall shear stress sensor for wall-bounded turbulent flows},
  author={Amili, O. and Soria, J.},
  journal={Exp. Fluids},
  volume={51},
  number={1},
  pages={137--147},
  year={2011},
  publisher={Springer}
}

@article{pastuhoff2013enhancing,
  title={Enhancing the signal-to-noise ratio of pressure sensitive paint data by singular value decomposition},
  author={Pastuhoff, M. and Yorita, D. and Asai, K. and Alfredsson, P. H.},
  journal={Meas. Sci. Tech.},
  volume={24},
  number={7},
  pages={075301},
  year={2013},
  publisher={IOP Publishing}
}

@article{gnanamanickam2013,
  title={Measurement of turbulent wall shear-stress using micro-pillars},
  author={E. P. Gnanamanickam and B. Nottebrock and S. Grotextbetae and J. P. Sullivan and W. Schroder},
  journal={Meas. Sci. Tech.},
  volume={24},
  number={12},
  pages={124002},
  year={2013},
  publisher={IOP Publishing}
}

@article{cattafesta2011actuators,
  title={Actuators for active flow control},
  author={Cattafesta, L. N and Sheplak, M.},
  journal={Annu. Rev. Fluid Mech.},
  volume={43},
  number={1},
  pages={247--272},
  year={2011},
  publisher={Annual Reviews}
}

@article{guastoni2024fully,
  title = {Fully convolutional networks for velocity-field predictions based on the wall heat flux in turbulent boundary layers},
  volume = {39},
  ISSN = {1432-2250},
  DOI = {10.1007/s00162-024-00732-y},
  number = {1},
  journal = {Theor. Comput. Fluid Dyn.},
  publisher = {Springer Science and Business Media LLC},
  author = {Guastoni,  L. and Balasubramanian,  A. G. and Foroozan,  F. and G\"{u}emes,  A. and Ianiro,  A. and Discetti,  S. and Schlatter,  P. and Azizpour,  H. and Vinuesa,  R.},
  year = {2024},
  month = dec 
}

@article{kerherve2017combining,
  title={Combining time-resolved multi-point and spatially-resolved measurements for the recovering of very-large-scale motions in high {R}eynolds number turbulent boundary layer},
  author={Kerherv{\'e}, F. and Roux, S. and Mathis, R.},
  journal={Exp. Therm. Fluid Sci.},
  volume={82},
  pages={102--115},
  year={2017},
  publisher={Elsevier}
}

@article{discetti2019characterization,
  title={{Characterization of very-large-scale motions in high-Re pipe flows}},
  author={Discetti, S. and Bellani, G. and {\"O}rl{\"u}, R. and Serpieri, J. and Sanmiguel Vila, C.  and Raiola, M. and Zheng, X. and Mascotelli, L. and Talamelli, A. and Ianiro, A.},
  journal={Exp. Therm. Fluid Sci.},
  volume={104},
  pages={1--8},
  year={2019},
  publisher={Elsevier}
}

@article{encinar2019logarithmic,
  title={Logarithmic-layer turbulence: a view from the wall},
  author={Encinar, M. P. and Jim{\'e}nez, J.},
  journal={Phys. Rev. Fluids},
  volume={4},
  number={11},
  pages={114603},
  year={2019},
  publisher={APS}
}

@article{cuellar2024some,
  title={{Some effects of limited wall-sensor availability on flow estimation with 3D-GANs}},
  author={Cu{\'e}llar, A. and Ianiro, A. and Discetti, S.},
  journal={Theor. Comput. Fluid Dyn.},
  pages={1--17},
  year={2024},
  publisher={Springer}
}

@article{cuellar2024three,
  title={Three-dimensional generative adversarial networks for turbulent flow estimation from wall measurements},
  author={Cu{\'e}llar, A. and G{\"u}emes, A. and Ianiro, A. and Flores, {\'O}. and Vinuesa, R. and Discetti, S.},
  journal={J. Fluid Mech.},
  volume={991},
  pages={A1},
  year={2024},
  publisher={Cambridge University Press}
}

@article{guastoni2021convolutional,
  title={Convolutional-network models to predict wall-bounded turbulence from wall quantities},
  author={Guastoni, L. and G{\"u}emes, A. and Ianiro, A. and D., Stefano and Schlatter, P. and Azizpour, H. and Vinuesa, R.},
  journal={J. Fluid Mech.},
  volume={928},
  pages={A27},
  year={2021},
  publisher={Cambridge University Press}
}

@article{guemes2021coarse,
  title={From coarse wall measurements to turbulent velocity fields through deep learning},
  author={G{\"u}emes, A. and Discetti, S. and Ianiro, A. and Sirmacek, B. and Azizpour, H. and Vinuesa, R.},
  journal={Phys. Fluids},
  volume={33},
  number={7},
  year={2021},
  publisher={AIP Publishing}
}

@article{guemes2019sensing,
  title={Sensing the turbulent large-scale motions with their wall signature},
  author={G{\"u}emes, A. and Discetti, S. and Ianiro, A.},
  journal={Phys. Fluids},
  volume={31},
  number={12},
  year={2019},
  publisher={AIP Publishing}
}

@article{Abe2001,
  title={Direct numerical simulation of a fully developed turbulent channel flow with respect to the Reynolds number dependence},
  author={Abe, H. and Kawamura, H. and Matsuo, Y.},
  journal={J. Fluids Eng.},
  volume={123},
  number={2},
  pages={382--393},
  year={2001}
}

@article{Abe2004,
title = {Surface heat-flux fluctuations in a turbulent channel flow up to {Re}$_\tau$=1020 with {Pr}=0.025 and 0.71},
author = {H. Abe and H. Kawamura and Y. Matsuo},
journal = {International J. Heat Fluid Fl.},
volume = {25},
number = {3},
pages = {404-419},
year = {2004},
issn = {0142-727X},
doi = {https://doi.org/10.1016/j.ijheatfluidflow.2004.02.010}
}

@article{Abe2009,
  title={Near-wall similarity between velocity and scalar fluctuations in a turbulent channel flow},
  author={Abe, H and Antonia, R. A.},
  journal={Phys. Fluids},
  volume={21},
  number={2},
  pages={025109},
  year={2009},
  publisher={American Institute of Physics}
}

@article{li2009dns,
  title={{DNS of a spatially developing turbulent boundary layer with passive scalar transport}},
  author={Li, Q. and Schlatter, P. and Brandt, L. and Henningson, D. S.},
  journal={International J. Heat Fluid Fl.},
  volume={30},
  number={5},
  pages={916--929},
  year={2009},
  publisher={Elsevier}
}

@article{balasubramanian2023direct,
  title={{Direct numerical simulation of a zero-pressure-gradient turbulent boundary layer with passive scalars up to Prandtl number Pr= 6}},
  author={Balasubramanian, A. G. and Guastoni, L. and Schlatter, P. and Vinuesa, R.},
  journal={J. Fluid Mech.},
  volume={974},
  pages={A49},
  year={2023},
  publisher={Cambridge University Press}
}

@Article{Batchelor59,
  author = 	 {G. K. Batchelor},
  title = 	 {Small-scale variation of convected quantities like temperature in turbulent fluid. Part 1. General discussion and the case of small conductivity.},
  journal = 	 {J.~Fluid Mech.},
  year = 	 {1971},
  volume = 	 {5},
  pages = 	 {113--133},
}

@Article{Brownell04,
  author = 	 {C. J. Brownell and L. K. Su},
  title = 	 {Planar measurements of differential diffusion in turbulent jets},
  journal = 	 {AIAA Paper 2004-2335},
  year = 	 {2004},
}

@Article{Brownell07,
  author = 	 {C. J. Brownell and L. K. Su},
  title = 	 {Scale relations and spatial spectra in a differentially diffusing jet},
  journal = 	 {AIAA Paper 2007-1314},
  year = {2007},
}

@InCollection{Dennis85,
  author = 	 {S. C. R. Dennis},
  title = 	 {{Compact explicit finite difference approximations to the Navier--Stokes equation}},
  booktitle = 	 {Ninth Intl Conf. on Numerical Methods in Fluid Dynamics},
  publisher = {Springer},
  year = 	 {1985},
  volume = 	 {218},
  series = 	 {Lecture Notes in Physics},
  pages = 	 {23--51},
}

@Article{Hwang70,
  author = 	 {L.-S. Hwang and E. O. Tuck},
  title = 	 {On the oscillations of harbours of arbitrary shape},
  journal = 	 {J.~Fluid Mech.},
  year = 	 {1970},
  volume = 	 {42},
  pages = 	 {447--464},
}

@InCollection{Worster92,
  author = 	 {M. G. Worster},
  title = 	 {{The dynamics of mushy layers}},
  booktitle = 	 {In Interactive dynamics of convection and solidification},
  publisher = {Kluwer},
  year = 	 {1992},
  editor = 	 {S. H. Davis and H. E. Huppert and W. Muller and M. G. Worster},
  pages = 	 {113--138},
}

@Article{Koch83,
  author = 	 {W. Koch},
  title = 	 {Resonant acoustic frequencies of flat plate cascades},
  journal = 	 {J.~Sound Vib.},
  year = 	 {1983},
  volume = 	 {88},
  pages = 	 {233--242},
}

@Article{Lee71,
  author = 	 {J.-J. Lee},
  title = 	 {Wave-induced oscillations in harbours of arbitrary geometry},
  journal = 	 {J.~Fluid Mech.},
  year = 	 {1971},
  volume = 	 {45},
  pages = 	 {375--394},
}

@Article{Linton92,
  author = 	 {C. M. Linton and D. V. Evans},
  title = 	 {The radiation and scattering of surface waves by a vertical circular cylinder in a channel},
  journal = 	 {Phil.\ Trans.\ R. Soc.\ Lond.},
  year = 	 {1992},
  volume = 	 {338},
  pages = 	 {325--357},
}

@Article{Martin80,
  author = {P. A. Martin},
  title =  {On the null-field equations for the exterior problems of acoustics},
  year ={1980},
  journal = {Q.~J. Mech.\ Appl.\ Maths},
  volume = {33},
  pages ={385--396},
}

@TechReport{Rogallo81,
   author = {R. S. Rogallo},
   title = {Numerical experiments in homogeneous turbulence},
   institution = {NASA Tech.\ Mem.},
   year = 1981,
   number = 81835
}

@Article{Ursell50,
  author = {F. Ursell},
  title = {Surface waves on deep water in the presence of a submerged cylinder I},
  year = {1950},
  journal = {Proc.\ Camb.\ Phil.\ Soc.}, 
  volume = {46},
  pages = {141--152}
}

@Article{Wijngaarden68,
  title = {On the oscillations near and at resonance in open pipes},
  author = {L. {van Wijngaarden}},
  year = {1968},
  journal = {J.~Engng Maths},
  volume = {2},
  pages = {225--240}
}

@PhdThesis{Miller91,
  title = {Mixing in high Schmidt number turbulent jets},
  author = {P. L. Miller},
  school = {California Institute of Technology},
  year = {1991},
  address = {}
}

@article{Krogstad1998ConvectionVI,
  title={Convection velocities in a turbulent boundary layer},
  author={P. Krogstad and J. H. Kaspersen and S. Rimestad},
  journal={Phys. Fluids},
  year={1998},
  volume={10},
  pages={949-957}
}

@book{smith2019turbulence,
  title={Turbulence: An introduction for scientists and engineers},
  author={Smith, L.M.},
  year={2019},
  publisher={Springer}
}

@book{smits2011turbulent,
  title={Turbulent shear layers in supersonic flow},
  author={Smits, A.J. and Dussauge, J.P.},
  year={2011},
  publisher={Cambridge University Press}
}

@article{adrian2007hairpin,
  title={Hairpin vortex organization in wall turbulence},
  author={Adrian, R.J.},
  journal={Phys. Fluids},
  volume={19},
  number={4},
  pages={041301},
  year={2007}
}

@article{dean1978reynolds,
  title={Reynolds-number dependence of skin friction and other bulk flow variables in two-dimensional rectangular duct flow},
  author={Dean, R.B.},
  journal={Journal of Fluids Engineering},
  volume={100},
  number={2},
  pages={215-223},
  year={1978}
}

@article{lee2015study,
  title={Study of wall turbulence using the linear stochastic estimation},
  author={Lee, M. and Kim, J.},
  journal={J. Fluid Mech.},
  volume={782},
  pages={474-506},
  year={2015}
}

@article{adrian1985large,
  title={Large eddy simulation of turbulent channel flow using subgrid scale closure},
  author={Adrian, R.J. and Yao, C.S.},
  journal={Phys. Fluids},
  volume={28},
  number={1},
  pages={010601},
  year={1985}
}

@book{gadelhak2000flow,
  title={Flow control: Passive, active, and reactive flow management},
  author={Gad-el-Hak, M.},
  year={2000},
  publisher={Cambridge University Press}
}

@article{haworth1986conditional,
  title={The conditional eddy-viscosity model applied to mixing in a round jet},
  author={Haworth, D.C. and Pope, S.B.},
  journal={J. Fluid Mech.},
  volume={170},
  pages={57-90},
  year={1986}
}

@article{rodriguez2013coherent,
  title={Coherent structure signatures of heat transfer in turbulent thermal boundary layers},
  author={Rodríguez, I. and Rodríguez, E. and Gutiérrez, E. and Serres, D.},
  journal={J. Fluid Mech.},
  volume={726},
  pages={285-318},
  year={2013}
}

@article{marusic2010predictive,
  title={Predictive model for wall-bounded turbulent flow},
  author={Marusic, I. and Mathis, R. and Hutchins, N.},
  journal={Science},
  volume={329},
  number={5988},
  pages={193-196},
  year={2010}
}

@article{Yamada2016,
  title="Construction of 2{D}-3{C} {PIV} and high-speed infrared thermography combined system for simultaneous measurement of flow and thermal fluctuations over a backward facing step",
  author="S. Yamada and H. Nakamura",
  journal="Int. J. Heat Fluid Fl.",
  year="2016",
  volume="61",
  pages="174-182"
}

@article{nakamura2013,
  title={Turbulence structure identification in a wall-bounded turbulent flow using infrared thermography},
  author={Nakamura, Y. and Yamada, H.},
  journal={J. Fluid Mech.},
  volume={735},
  pages={332--358},
  year={2013},
  publisher={Cambridge University Press}
}

@article{foroozan2023,
  title={Synchronized measurement of instantaneous convective heat flux and velocity fields in wall-bounded flows},
  author={Foroozan, F. and G{\"u}emes, A. and Raiola, M. and Castellanos, R. and Discetti, S. and Ianiro, A.},
  journal={Meas. Sci. Tech.},
  volume={34},
  number={12},
  pages={125301},
  year={2023},
  publisher={IOP Publishing}
}

@article{adrian1985,
  title={Stochastic estimation of conditional structure: A review},
  author={Adrian, R.J. and Yao, C.S.},
  journal={Exp. Fluids},
  volume={7},
  number={8},
  pages={323--335},
  year={1985},
  publisher={Springer}
}

@article{delalamo2004,
  title={Scaling of the energy spectra of turbulent channels},
  author={del {\'A}lamo, J.C. and Jim{\'e}nez, J.},
  journal={J. Fluid Mech.},
  volume={500},
  pages={135--144},
  year={2004},
  publisher={Cambridge University Press}
}

@article{DELÁLAMO_JIMÉNEZ_2009,
  title={Estimation of turbulent convection velocities and corrections to {T}aylor’s approximation},
  author={Del {\'A}lamo, J.C. and Jim{\'e}nez, J.},
  volume={640},
  DOI={10.1017/S0022112009991029},
  journal={J. Fluid Mech.},
  year={2009},
  pages={5–26}
}

@article{MOIN_2009,
  title={Revisiting {T}aylor’s hypothesis},
  author={Moin, P.},
  volume={640},
  DOI={10.1017/S0022112009992126},
  journal={J. Fluid Mech.},
  year={2009},
  pages={1–4}
}

@article{Choi1990,
  title = {On the space-time characteristics of wall-pressure fluctuations},
  author = {Choi,  H. and Moin,  P.},
  volume = {2},
  ISSN = {0899-8213},
  DOI = {10.1063/1.857593},
  number = {8},
  journal = {Phys. Fluids A: Fluid},
  publisher = {AIP Publishing},
  year = {1990},
  month = aug,
  pages = {1450–1460}
}

@article{goldschmidt_young_ott_1981,
  title={Turbulent convective velocities (broadband and wavenumber dependent) in a plane jet},
  author={Goldschmidt, V. W. and Young, M. F. and Ott, E. S.},
  volume={105},
  DOI={10.1017/S0022112081003236},
  journal={J. Fluid Mech.},
  publisher={Cambridge University Press},
  year={1981},
  pages={327–345}
}

@article{wills_1964, 
  title={On convection velocities in turbulent shear flows}, 
  author={Wills, J. A. B.}, 
  volume={20}, 
  DOI={10.1017/S002211206400132X}, 
  number={3}, 
  journal={J. Fluid Mech.}, 
  publisher={Cambridge University Press}, 
  year={1964}, 
  pages={417–432}
}

@article{Kline1967,
  title={The structure of turbulent boundary layers},
  author={Kline, S. J. and Reynolds, W. C. and Schraub, F. A. and Runstadler, P. W.},
  volume={30},
  DOI={10.1017/S0022112067001740},
  number={4},
  journal={J. Fluid Mech.},
  year={1967},
  pages={741–773}
}

@article{Smits2011,
   author = "Smits, A. J. and McKeon, B. J. and Marusic, I.",
   title = "High–{R}eynolds Number Wall Turbulence", 
   journal= "Annu. Rev. Fluid Mech.",
   year = "2011",
   volume = "43",
   number = "Volume 43, 2011",
   pages = "353-375",
   doi = "https://doi.org/10.1146/annurev-fluid-122109-160753",
   publisher = "Annual Reviews"
  }

@article{Smith_Metzler_1983,
title={The characteristics of low-speed streaks in the near-wall region of a turbulent boundary layer},
author={Smith, C. R. and Metzler, S. P.},
volume={129},
DOI={10.1017/S0022112083000634},
journal={J. Fluid Mech.},
year={1983},
pages={27–54}
}

@article{Klewicki1995,
    author = {Klewicki, J. C. and Metzger, M. M. and Kelner, E. and Thurlow, E. M.},
    title = "{Viscous sublayer flow visualizations at {$\mathbf{R}_\theta\approx1.500.000$}}",
    journal = {Phys. Fluids},
    volume = {7},
    number = {4},
    pages = {857-863},
    year = {1995},
    month = {04},
    issn = {1070-6631},
    doi = {10.1063/1.868763}
}

@article{RAIOLA2017,
    title = {Towards enabling time-resolved measurements of turbulent convective heat transfer maps with IR thermography and a heated thin foil},
    author = {M. Raiola and C. S. Greco and M. Contino and S. Discetti and A. Ianiro},
    journal = {Int. J. Heat Mass Tran.},
    volume = {108},
    pages = {199-209},
    year = {2017},
    issn = {0017-9310},
    doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2016.12.002},
}

@article{NAKAMURA2009,
    title = {Frequency response and spatial resolution of a thin foil for heat transfer measurements using infrared thermography},
    author = {H. Nakamura},
    journal = {Int. J. Heat Mass Tran.},
    volume = {52},
    number = {21},
    pages = {5040-5045},
    year = {2009},
    issn = {0017-9310},
    doi = {https://doi.org/10.1016/j.ijheatmasstransfer.2009.04.019},
}

@article{Dacome2024,
  title = {Opposition flow control for reducing skin-friction drag of a turbulent boundary layer},
  author = {Dacome, G. and M\"orsch, R. and Kotsonis, M. and Baars, W. J.},
  journal = {Phys. Rev. Fluids},
  volume = {9},
  issue = {6},
  pages = {064602},
  numpages = {27},
  year = {2024},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevFluids.9.064602},
}

@article{Sillero2013,
  title = {{One-point statistics for turbulent wall-bounded flows at Reynolds numbers up to $\delta^+ \approx 2000$}},
  volume = {25},
  ISSN = {1089-7666},
  DOI = {10.1063/1.4823831},
  number = {10},
  journal = {Phys. Fluids},
  publisher = {AIP Publishing},
  author = {Sillero,  J. A. and Jiménez,  J. and Moser,  R. D.},
  year = {2013},
  month = oct 
}

@article{Sillero2014,
  title = {{Two-point statistics for turbulent boundary layers and channels at Reynolds numbers up to $\delta^+ \approx 2000$}},
  volume = {26},
  ISSN = {1089-7666},
  DOI = {10.1063/1.4899259},
  number = {10},
  journal = {Phys. Fluids},
  publisher = {AIP Publishing},
  author = {Sillero,  Juan A. and Jiménez,  Javier and Moser,  Robert D.},
  year = {2014},
  month = oct 
}

@article{Baars_Dacome_Lee_2024,
    title={Reynolds-number scaling of wall-pressure–velocity correlations in wall-bounded turbulence}, 
    author={Baars, W. J. and Dacome, G. and Lee, M.},
    volume={981},
    DOI={10.1017/jfm.2024.46},
    journal={J. Fluid Mech.},
    year={2024},
    pages={A15}
}

@article{Taylor1938,
    author = {Taylor, G. I. },
    title = {The Spectrum of Turbulence},
    journal = {P. Roy. Soc. A-Math. Phy.},
    volume = {164},
    number = {919},
    pages = {476-490},
    year = {1938},
    doi = {10.1098/rspa.1938.0032},
}

@article{Miozzi2024,
  author = {M. Miozzi and A. Schr\"{o}der and D. Schanz and C. E. Willert and C. Klein and J. Lemarechal},
  title = {Skin-friction from temperature and velocity data around a wall-mounted cube},
  volume = {65},
  ISSN = {1432-1114},
  DOI = {10.1007/s00348-024-03881-2},
  number = {10},
  journal = {Exp. Fluids},
  publisher = {Springer Science and Business Media LLC},
  year = {2024},
  month = oct 
}

@article{Kim1993,
  title = {Propagation velocity of perturbations in turbulent channel flow},
  volume = {5},
  ISSN = {0899-8213},
  DOI = {10.1063/1.858653},
  number = {3},
  journal = {Phys. Fluids A: Fluid},
  publisher = {AIP Publishing},
  author = {J. Kim and F. Hussain},
  year = {1993},
  month = mar,
  pages = {695–706}
}

@article{Jeon1999,
  title = {Space–time characteristics of the wall shear-stress fluctuations in a low-Reynolds-number channel flow},
  author = {Jeon,  S. and Choi,  H. and Yoo,  J. Y. and Moin,  P.},
  volume = {11},
  ISSN = {1089-7666},
  DOI = {10.1063/1.870166},
  number = {10},
  journal = {Phys. Fluids},
  publisher = {AIP Publishing},
  year = {1999},
  month = oct,
  pages = {3084–3094}
}

@article{Cui_Jacobi_2024,
    title={Variability of convection velocities and structure inclination angles in wall-bounded turbulence},
    volume={989},
    DOI={10.1017/jfm.2024.518},
    journal={J. Fluid Mech.},
    author={Cui, G. and Jacobi, I.},
    year={2024},
    pages={A16}
}

@article{Cattell1966,
    author = {R. B. Cattell},
    title = {The Scree Test For The Number Of Factors},
    journal = {Multiv. Behav. Res.},
    volume = {1},
    number = {2},
    pages = {245--276},
    year = {1966},
    publisher = {Routledge},
    doi = {10.1207/s15327906mbr0102\_10}
}

@article{MOFFAT19883,
    author = {R. J. Moffat},
    title = {Describing the uncertainties in experimental results},
    journal = {Exp. Therm. Fluid Sci.},
    volume = {1},
    number = {1},
    pages = {3-17},
    year = {1988},
}

@article{SCHULTZ_FLACK_2007, 
    title={The rough-wall turbulent boundary layer from the hydraulically smooth to the fully rough regime}, 
    volume={580}, 
    DOI={10.1017/S0022112007005502}, 
    journal={J. Fluid Mech.}, 
    author={Schultz, M. P. and Flack, K. A.}, 
    year={2007}, 
    pages={381–405}
}

@article{Liu_Gayme_2020, 
title={An input–output based analysis of convective velocity in turbulent channels}, 
volume={888}, 
DOI={10.1017/jfm.2020.48}, 
journal={J. Fluid Mech.}, 
author={Liu, Chang and Gayme, Dennice F.}, 
year={2020}, 
pages={A32}
}

@article{mcadams1926heat,
  title={Heat transmission from condensing steam to water in surface condensers and feedwater heaters},
  author={McAdams, WH and Sherwood, TK and Turner, RL},
  journal={J. Fluids Eng.},
  volume={48},
  pages={1233--1258},
  year={1926},
  publisher={American Society of Mechanical Engineers Digital Collection}
}

@article{Taler2017,
  title = {Simple power-type heat transfer correlations for turbulent pipe flow in tubes},
  volume = {26},
  ISSN = {1993-033X},
  DOI = {10.1007/s11630-017-0947-2},
  number = {4},
  journal = {J. Thermal Sci.},
  publisher = {Springer Science and Business Media LLC},
  author = {Taler,  Dawid},
  year = {2017},
  month = jul,
  pages = {339–348}
}

@article{Sieder1936HeatTA,
  title={Heat Transfer and Pressure Drop of Liquids in Tubes},
  author={E. N. Sieder and G. E. Tate},
  journal={Ind. Eng. Chem.},
  year={1936},
  volume={28},
  pages={1429-1435}
}
